Non-Abelian lattice gauge fields in the photonic synthetic frequency dimension

Non-Abelian gauge fields provide a conceptual framework for the description of particles having spins. The theoretical importance of non-Abelian gauge fields motivates their experimental synthesis and explorations. Here, we demonstrate non-Abelian lattice gauge fields for photons. In the study of gauge fields, lattice models are essential for the understanding of their implications in extended systems. We utilize the platform of synthetic frequency dimensions, which enables the study of lattice physics in a scalable and programmable way. We observe Dirac cones at time-reversal-invariant momenta as well as the direction reversal of eigenstate trajectories associated with such Dirac cones. Both of them are unique signatures of non-Abelian gauge fields in our lattice system. Our results highlight the implications of non-Abelian gauge field in the study of topological physics and suggest opportunities for the control of photon spins and pseudospins.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
